DeAR: Fine-Grained VLM Adaptation by Decomposing Attention Head Roles

Prompt learning is a dominant paradigm for adapting pre-trained Vision-Language Models (VLMs) to downstream tasks. However, existing methods often rely on a simplistic, layer-centric view, assuming shallow layers capture general features while deep layers handle task-specific knowledge. This assumption results in uncontrolled interactions between learnable tokens and original tokens. Task-specific knowledge could degrades the model's core generalization and creates a trade-off between task adaptation and the preservation of zero-shot generalization. To address this, we challenge the layer-centric view and propose \textbf{DeAR}, a framework that achieves fine-grained VLM adaptation by \textbf{De}composing \textbf{A}ttention head \textbf{R}oles. We posit that the functional specialization within VLMs occurs not between layers, but at the finer-grained level of individual attention heads in the deeper layers. Based on this insight, we introduce a novel metric, Concept Entropy, to systematically classify attention heads into distinct functional roles: \textit{Attribute}, \textit{Generalization}, and \textit{Mixed}. Guided by these roles, we introduce specialized attribute tokens and a Role-Based Attention Mask mechanism to precisely control information flow, ensuring generalization heads remain isolated from task-specific knowledge. We further incorporate a Task-Adaptive Fusion Strategy for inference. Extensive experiments on fifteen datasets show that DeAR achieves a strong balance between task adaptation and generalization, outperforming previous methods across various tasks.

==> sec/0_abstract.tex <==
\begin{abstract}
Prompt learning is a dominant paradigm for adapting pre-trained Vision-Language Models (VLMs) to downstream tasks. However, existing methods often rely on a simplistic, layer-centric view, assuming shallow layers capture general features while deep layers handle task-specific knowledge. This assumption results in uncontrolled interactions between learnable tokens and original tokens. Task-specific knowledge could degrade the model's core generalization and creates a trade-off between task adaptation and the preservation of zero-shot generalization. To address this, we challenge the layer-centric view and propose \textbf{DeAR}, a framework that achieves fine-grained VLM adaptation by \textbf{De}composing \textbf{A}ttention head \textbf{R}oles. We posit that the functional specialization within VLMs occurs not between layers, but at the finer-grained level of individual attention heads in the deeper layers. Based on this insight, we introduce a novel metric, Concept Entropy, to systematically classify attention heads into distinct functional roles: \textit{Attribute}, \textit{Generalization}, and \textit{Mixed}. Guided by these roles, we introduce specialized attribute tokens and a Role-Based Attention Mask mechanism to precisely control information flow, ensuring generalization heads remain isolated from task-specific knowledge. We further incorporate a Task-Adaptive Fusion Strategy for inference. Extensive experiments on fifteen datasets show that DeAR achieves a strong balance between task adaptation and generalization, outperforming previous methods across various tasks. Our code is available at \url{https://github.com/wellsssssss/DeAR}
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}

Pre-trained Vision-Language Models (VLMs), such as CLIP \citep{radford2021learningtransferablevisualmodels}, have emerged as a new paradigm in computer vision, demonstrating remarkable zero-shot generalization capabilities across a wide range of downstream tasks. By leveraging contrastive learning on over 400 million image-text pairs, CLIP learns to align visual and textual inputs in a shared embedding space. This has led to impressive achievements in tasks such as text-image retrieval \citep{radford2021learningtransferablevisualmodels}, visual question answering (VQA) \citep{gao2025clipadapterbettervisionlanguagemodels}, and open-vocabulary detection and segmentation \citep{gu2022openvocabularyobjectdetectionvision,Wang_Chen_Kang_Li_Xian_Chen_Xu_2025}. Moreover, the impact of CLIP extends to traditional vision tasks, such as image classification and object detection \citep{9879567}, where its zero-shot performance can surpass that of fully supervised methods.

Despite these successes, adapting CLIP to specific downstream tasks remains a significant challenge. Its pre-trained knowledge often lacks the granularity required for specialized domains. Although full fine-tuning could incorporate this new knowledge, it is computationally expensive and often leads to "catastrophic forgetting," where the model loses its powerful zero-shot generalization abilities \citep{kirkpatrick2017overcoming}. Consequently, Parameter-Efficient Fine-Tuning (PEFT) methods have become the mainstream approach \citep{wang2024megafaketheorydrivendatasetfake, liu2025sara}. These methods keep the VLM backbone frozen and introduce a small number of trainable parameters. PEFT strategies include adapter-based methods and prompt learning. The former typically insert lightweight MLP layers to refine the output features \citep{seputis2024multimodaladaptervisionlanguagemodels,gao2025clipadapterbettervisionlanguagemodels,zhu2023featuresmatterenhancingfewshot}, while prompt learning has emerged as a dominant and effective paradigm.

\begin{figure}[t]
    \centering
    % Placeholder for the framework figure
    \includegraphics[width=0.5\textwidth]{author-kit-CVPR2026-v1-latex-/sec/compare_cropped.pdf}
    \caption{For a Generalization Head (e.g., Layer 9 Head 0), our Role-Based Mask explicitly blocking the original CLS and Patch tokens from interacting to the inserted Attribute Tokens.}
    \label{fig:compare}
\end{figure}

Prompt learning for VLMs was pioneered by CoOp \citep{Zhou_2022}, which introduced "soft prompts" , learnable continuous vectors, into the text encoder to adapt to downstream tasks. Subsequent work extended this concept to the vision domain, with VPT \citep{jia2022visualprompttuning} demonstrating the effectiveness of visual prompting. A key breakthrough came with MaPLe \citep{khattakMaPLe}, which proposed the first multi-modal prompt learning framework, tuning prompts in both the vision and text encoders and proving its superiority over uni-modal approaches.

However, even with a frozen backbone, prompt learning methods still risk losing generalization capabilities. Due to the nature of the Vision Transformer \citep{dosovitskiy2021imageworth16x16words,vaswani2023attentionneed}, inserted tokens inevitably interact with original tokens via multi-head self-attention, which can harm generalization. Existing solutions attempt to address this by carefully selecting which layers to inject prompts into—some targeting early layers (MaPLe), while others target deeper ones (MMRL). These conflicting, layer-based strategies reveal a fundamental gap: they treat entire Transformer layers as black boxes, ignoring the diverse functional roles played by individual attention heads within them. This lack of a fine-grained, principled approach for integrating new knowledge results in the challenging trade-off between achieving effective adaptation and maintaining generalization.

% However, even with a frozen backbone, prompt learning's effectiveness is hampered by a critical vulnerability: the uncontrolled interaction between inserted prompts and original tokens within the self-attention mechanism \citep{dosovitskiy2021imageworth16x16words,vaswani2023attentionneed}, which can corrupt the model's pre-trained knowledge \citep{wang2024megafaketheorydrivendatasetfake, liu2025sara}. This vulnerability stems from a flawed, layer-centric assumption that functional roles are neatly stratified across layers. This has led to conflicting and heuristic strategies—some methods prompt early layers (e.g., MaPLe), while others target deep layers (e.g., MMRL). The lack of consensus reveals a fundamental gap: existing methods treat the internal workings of Transformer blocks as opaque, lacking a principled way to integrate new knowledge without causing catastrophic forgetting.




To address these challenges, we draw inspiration from recent work on VLM interpretability \citep{gandelsman2024interpreting} and propose a novel framework: \textbf{DeAR}, a novel framework for fine-grained VLM adaptation achieved by \textbf{De}composing \textbf{A}ttention head \textbf{R}oles. Given that CLIP's final image representation is constructed by its late attention layers, we suppose that the key to effective task adaptation, while preserving generalization, is to focus on the functional specialization of these individual heads.  Our approach begins by quantitatively analyzing the function of each attention head in the later layers of a ViT-B-16 backbone \citep{dosovitskiy2021imageworth16x16words}. Using our proposed Concept Entropy metric, we classify these heads into distinct functional roles: Attribute Heads, Generalization Heads, and Mixed Heads. Leveraging this functional classification, DeAR introduces specialized, learnable attribute tokens and employs a role-based Attention Mask strategy. This mechanism precisely controls the information flow, guiding attribute tokens to interact primarily with their corresponding expert heads, while critically isolating the generalization heads from any new task-specific knowledge (Figure~\ref{fig:compare}). Our contributions are as follows:
\begin{itemize}
    \item We introduce \textbf{Concept Entropy}, a novel quantitative metric to systematically analyze and classify the functional roles of attention heads in ViT-B/16, revealing a clear specialization into Attribute, Generalization, and Mixed roles.
    \item We propose the \textbf{DeAR}, which introduces a Role-Based Attention Mask to leverage this functional map. This mechanism achieves controllable fine-tuning by precisely routing new knowledge to expert heads while shielding generalization heads, achieving a balance between task-specific adaptation and the preservation of generalization capabilities.
    \item We demonstrate through extensive experiments that DeAR achieves \textbf{new state-of-the-art performance} on the challenging base-to-novel generalization benchmark.
\end{itemize}

==> sec/2_related_work.tex <==
\section{Related Work}

\subsection{Vision-Language Models (VLMs)}
Foundational Vision-Language Models (VLMs) have revolutionized multimodal learning. This paradigm was pioneered by CLIP \citep{radford2021learningtransferablevisualmodels}, which established a powerful contrastive learning framework on massive web-scale data. Subsequent efforts have expanded on this foundation in diverse ways: ALIGN \citep{pmlr-v139-jia21b} demonstrated the power of training on even larger, noisier datasets; Florence \citep{yuan2021florencenewfoundationmodel} aimed for a universal visual representation via multi-task pre-training; SigLIP \citep{10377550} enhanced scalability with a simpler pairwise sigmoid loss; and more recently, OpenVision \citep{li2025openvisionfullyopencosteffectivefamily} has proposed full transparency by leveraging high-quality, LLM-generated synthetic captions.

\subsection{Prompt Learning for VLMs}
Prompt learning has emerged as a dominant parameter-efficient strategy for adapting VLMs. The line of research was pioneered by CoOp, which replaces hand-crafted templates with learnable prompt vectors\citep{Zhou_2022}. However, CoOp learns a single static prompt for the entire dataset, which tends to overfit seen classes and lacks adaptability to individual images. Subsequent studies proposed CoCoOp, which conditions prompts on each image, and Task-Aware Clustering, which learns cluster-specific prompts for semantic subgroups\citep{zhou2022cocoop,Hao_2025_CVPR}. To preserve the general knowledge of the backbone, PromptSRC, ProGrad and TCP introduce various regularization techniques\citep{Khattak_2023_ICCV,https://doi.org/10.48550/arxiv.2205.14865,TCP24}.

As research matured, the focus expanded from uni-modal text prompts toward multimodal strategies. MaPLe presents a framework for simultaneous prompting in both vision and language branches\citep{khattakMaPLe}, and more recent work such as MMRL designs shared representation spaces to facilitate deeper cross-modal interactions\citep{guo2025mmrl}. The latest trend pursues fine-grained semantics: LLaMP employs LLMs as adaptive prompt learners, ATPrompt constructs hybrid attribute--category prompt structures, PromptKD exploits prompts for knowledge distillation, and TextRefiner mines internal visual knowledge of VLMs to refine prompts without external models\citep{Zheng_2024_Large,li2025advancing,li2024promptkd,xie2024textrefinerinternalvisualfeature}. Alternatively, Skip Tuning forgoes additional parameters altogether and instead modifies the full fine-tuning baseline with layer-wise and class-wise skipping to improve knowledge transfer \citep{wu2024skip}.

\begin{figure*}[t]
    \centering
    % Placeholder for the framework figure
    \includegraphics[width=0.82\textwidth]{author-kit-CVPR2026-v1-latex-/sec/framework_cropped.pdf}
    \caption{The overall framework of DeAR. At a deep layer $J$, we insert learnable attribute tokens into the frozen vision encoder and the text encoder. Information flow in these subsequent layers is precisely controlled by our Role-Based Attention Mask mechanism. For inference, the class feature (from the \texttt{[CLS]} token) and attribute feature first compute the logits with the text feature. These logits are then combined via learnable fusion weights to produce the final prediction.}
    \label{fig:framework}
\end{figure*}



==> sec/3_method.tex <==
\section{Method}
Despite advances in VLMs and prompt learning, efficiently adapting these models while maintaining generalization is still challenging. Most existing methods focus on designing representation spaces or using prompts to inject external knowledge, but rarely explore how internal information flows within the model. Our work, DeAR, addresses this by directly investigating these internal interactions to enable attribute-aware and interpretable prompt learning.
% Our proposed A-Prompt framework is built upon the internal architecture of the Vision Transformer (ViT) \citep{dosovitskiy2021imageworth16x16words}, which serves as the image encoder in CLIP. To lay the groundwork for our method, we first revisit the key computational steps of ViT, detailing how an input image is processed into a final class representation.
\subsection{Revisiting the Vision Transformer}
\label{sec:preliminaries}



The ViT-based image encoder first converts an image into a sequence of patch embeddings. An input image $\mathbf{x}$ is divided into $N$ patches, which are linearly projected into $D$-dimensional vectors. A learnable \texttt{[CLS]} token, $\mathbf{z}_{\text{cls}}$, is prepended to this sequence, and position embeddings $\mathbf{E}_{\text{pos}}$ are added to yield the initial token sequence $\mathbf{z}^0 \in \mathbb{R}^{(N+1) \times D}$.

% This sequence is then processed by a stack of $L$ Transformer layers. Each layer consists of a Multi-Head Self-Attention (MSA) module and a feed-forward MLP, with residual connections and layer normalization. The MSA mechanism, which is central to our work, allows tokens to interact through $h$ parallel "attention heads." The output of the MSA module is a combination of the outputs of all heads:
% \begin{equation}
%     \text{MSA}(\mathbf{z}) = \text{Concat}(\text{head}_1, \dots, \text{head}_h) \mathbf{W}_o
%     \label{eq:msa_concat}
% \end{equation}
% where $\mathbf{W}_o$ is a final projection layer, and each individual head is computed via scaled dot-product attention:
% \begin{equation}
%     \text{head}_i = \text{softmax}\left(\frac{\mathbf{Q}_i\mathbf{K}_i^T}{\sqrt{D_h}}\right) \mathbf{V}_i
%     \label{eq:single_head_attention}
% \end{equation}

This sequence is then processed by a stack of $L$ Transformer layers. Each layer consists of a Multi-Head Self-Attention (MSA) module and a feed-forward MLP, with residual connections and layer normalization. Central to our work, the MSA mechanism allows tokens to interact through $h$ parallel "attention heads." The MSA module's output is computed by concatenating the outputs of all heads, i.e., $\text{MSA}(\mathbf{z}) = \text{Concat}(\text{head}_1, \dots, \text{head}_h)\mathbf{W}_o$, where $\mathbf{W}_o$ is a final projection layer. Each individual head is computed via scaled dot-product attention:
\begin{equation}
\text{head}_i = \text{softmax}\left(\frac{\mathbf{Q}_i\mathbf{K}_i^T}{\sqrt{D_h}}\right) \mathbf{V}_i
\label{eq:single_head_attention}
\end{equation}





\input{author-kit-CVPR2026-v1-latex-/sec/head_roles}




The Query ($\mathbf{Q}_i$), Key ($\mathbf{K}_i$), and Value ($\mathbf{V}_i$) matrices for each head $i$ are learned linear projections of the input tokens $\mathbf{z}$ using per-head weight matrices $(\mathbf{W}_{qi}, \mathbf{W}_{ki}, \mathbf{W}_{vi})$. 
After passing through all $L$ layers, the final state of the class token, $\mathbf{z}_{\text{cls}}^L$, is projected to yield the final image feature $\mathbf{f}_{\text{cls}}$. This multi-head self-attention mechanism forms the foundation of our controllable fine-tuning framework.


\subsection{Identifying Functional Roles of Attention Heads}
\label{sec:head_roles}

The core of DeAR is our hypothesis, inspired by recent interpretability studies \citep{gandelsman2024interpreting}, that the functional specialization of a VLM resides not at the layer level, but within individual attention heads in the model's deeper layers \citep{10.5555/3540261.3541188}. We propose a novel, unsupervised methodology to first \textit{identify} and then \textit{quantify} the functional roles of these heads \citep{vig-belinkov-2019-analyzing}. Our analysis focuses on the later layers (9--12) of ViT-B-16, which are known to be critical for constructing the final image representation.

To avoid subjective, pre-defined attribute categories, we adopt an approach to automatically identify conceptual clusters from the heads' description. Following \citet{gandelsman2024interpreting}, we first use TEXTSPAN to generate a ranked list of top-$N$ descriptive text phrases for each attention head. This yields a rich corpus of phrases describing each head's attentional focus. We then employ a pre-trained SBERT, $S(\cdot)$ \citep{reimers-gurevych-2019-sentence}, to map each phrase into a high-dimensional semantic space. Instead of classifying these phrase embeddings into a fixed set of categories, we perform density-based clustering using HDBSCAN \citep{mcinnes2017hdbscan}, a robust algorithm that can discover clusters of varying shapes and densities without requiring a pre-specified number of clusters. This automated process reveals a diverse set of conceptual clusters directly from the data. 

Our clustering analysis revealed 12 distinct conceptual groups, including concepts such as \textit{location}, \textit{text}, \textit{object}, \textit{animal}, \textit{photographic style}, and \textit{emotion}, etc. From these, we selected five frequent and semantically orthogonal concepts most relevant for general visual recognition tasks: $A = \{\texttt{color}, \texttt{shape}, \texttt{texture}, \texttt{object}, \texttt{location}\}$. This process provides the conceptual basis for our subsequent analysis, where the centroid of each selected cluster $c_j$ is denoted by its embedding $\bar{\mathbf{s}}_j = S(c_j)$.

\paragraph{Quantifying Specialization with Concept Entropy.}
With the core attributes established, we introduce a novel metric, \textbf{Concept Entropy}, to quantify the degree of functional specialization for each attention head $(l,h)$. For its top-$N$ descriptive phrases $D_{(l,h)}$, we first classify each phrase $d_i$ to the closest attribute cluster $c_j \in C$. This yields a probability distribution $P_{(l,h)}$ over the attributes, where $P_{(l,h)}(c_j)$ is the fraction of phrases assigned to $c_j$. Finally, the Concept Entropy $H(P_{(l,h)})$ is the Shannon entropy of this distribution. These steps are defined as:
\begin{gather}
    \text{cat}(d_i) = \arg\max_{c_j \in C} \cos\big(S(d_i), \bar{\mathbf{s}}_j\big) \\
    P_{(l,h)}(c_j) = \frac{1}{N} \sum\nolimits_{i=1}^{N} \mathbb{I}\big(\text{cat}(d_i) = c_j\big) \label{eq:prob_dist} \\ 
    H(P_{(l,h)}) = -\sum\nolimits_{j=1}^{k} P_{(l,h)}(c_j) \log_2 P_{(l,h)}(c_j)
\end{gather}
where $\mathbb{I}(\cdot)$ is the indicator function.
A low Concept Entropy score signifies that a head is highly specialized, concentrating its function on a single core attribute (\textbf{Attribute Head}). Conversely, a high score indicates a generalist function, engaging with a wide range of abstract concepts (\textbf{Generalization Head}). Heads with intermediate scores are classified as \textbf{Mixed Heads}. This role identification framework forms the foundation for DeAR's controllable learning mechanism.
% The foundation of our A-Prompt is built on the suppose that the attention heads within ViT possess functional specializations. To improve traditional prompt learning paradigm, we first explore the attention heads in the later layers of ViT-B-16, as these layers are known to be more critical for constructing the final image representation.

% Following the methodology proposed by \citet{gandelsman2024interpreting}, we use TEXTSPAN to generate a ranked list of top-20 descriptive text phrases for each attention head. Qualitative analysis of these descriptions reveals distinct functional roles. As illustrated in Table~\ref{tab:attribute_head_examples_wide}, some heads consistently focus on a single, concrete visual attribute. For instance, Layer 12, Head 10 is unequivocally a \textbf{Color Head}, with its top descriptions revolving around color terms.



% To quantify this functional specialization, we introduce a novel metric \textbf{Concept Entropy}. This metric measures the conceptual diversity within a head's descriptions. The process is as follows:
% First, we define a set of $k$ core visual attribute categories, $C = \{c_1, \dots, c_k\}$. For each head $(l,h)$, we consider its top $N$ descriptive phrases, $D_{(l,h)} = \{d_1, \dots, d_N\}$. We then use a pre-trained sentence transformer \citep{reimers-gurevych-2019-sentence}, $S(\cdot)$, to perform zero-shot classification of each phrase into one of the attribute categories. This model is chosen for its ability to map sentences to a dense vector space where semantic similarity directly corresponds to cosine similarity, making it highly effective for such zero-shot semantic matching tasks. The predicted category for a phrase $d_i$ is determined by maximum cosine similarity:
% % For efficiency, the category embeddings $S(c_j)$ are pre-computed once. 

% \begin{equation*}
% \label{eq:classify}
% \text{cat}(d_i) = \arg\max_{c_j \in C} \cos\big(S(d_i), S(c_j)\big)
% \end{equation*}

% This allows us to compute a discrete probability distribution $P_{(l,h)}$ over the categories for each head, where the probability of a category $c_j$ is the fraction of top-$N$ phrases classified into it:
% \[
% \label{eq:distribution}
% P_{(l,h)}(c_j) = \frac{1}{N} \sum_{i=1}^{N} \mathbb{I}\big(\text{cat}(d_i) = c_j\big)
% \]
% where $\mathbb{I}(\cdot)$ is the indicator function. Finally, the Concept Entropy $H(P_{(l,h)})$ for the head is calculated as the Shannon entropy of this distribution:
% \[
% \label{eq:entropy}
% H(P_{(l,h)}) = -\sum_{j=1}^{k} P_{(l,h)}(c_j) \log_2 P_{(l,h)}(c_j)
% \]
% A low Concept Entropy score indicates that a head is highly specialized, concentrating its function on a single attribute (\textbf{Attribute Head}). Conversely, a high score suggests a generalized function, engaging with a wide range of abstract concepts like artistic style or composition (\textbf{Generalization Head}). Heads with intermediate entropy scores are classified as \textbf{Mixed Head}. These heads often attend to a diverse set of concrete objects or scenes, demonstrating a broader but less abstract focus than the high-level concepts captured by Generalization Heads. We performed this analysis for all attention heads in layers 9 to 12 of ViT-B-16, with detailed classification results provided in the Appendix. These functional roles of attention head forms the foundation for our A-Prompt framework.
% % which we detail in the following section.


\subsection{DeAR: Fine-Grained Attribute-Aware Prompt Learning}
\label{sec:a_prompt_framework}

Building on our function analysis of attention heads, we introduce DeAR, a framework consisting of three key components: multimodal attribute-aware prompt learning, a role-based attention mask mechanism, and a task-adaptive inference strategy. The overall framework is shown in Figure~\ref{fig:framework}.
% a framework designed for precise, attribute-aware prompt learning. A-Prompt steers new information to specialized attribute heads while rigorously protecting the generalization capabilities of the CLIP. 


\subsubsection{Multimodal Attribute-Aware Prompting}
To adapt CLIP for downstream tasks, DeAR introduces learnable tokens into both the vision and text encoders, ensuring new knowledge is aligned across modalities.

\paragraph{Vision-Side Prompting.}
We initialize a set of learnable "attribute tokens," $\{\mathbf{r}_{\text{attr}} \in \mathbb{R}^{D_v}\}_{\text{attr} \in A}$, where $D_v$ is the feature dimension of the vision encoder. Here, $A$ is the set of core visual attributes identified in our analysis, specifically $A = \{\text{color}, \text{shape}, \text{texture}, \text{object}, \text{location}\}$. Based on the findings of \citet{gandelsman2024interpreting} that the final image representation in CLIP is predominantly constructed by the later attention layers, these attribute tokens are integrated into the higher layers of the image encoder $\mathcal{V}$, beginning from the $J$-th layer (we set $J$ = 9 in our experiments, following prior work on ViT analysis).

For the image encoder $\mathcal{V}$, the forward pass through the first $J-1$ layers proceeds as standard:
\begin{align*}
    [\mathbf{z}_{\text{cls}}^{\ell}, \mathbf{z}_{p}^{\ell}] &= \mathcal{V}_{\ell}([\mathbf{z}_{\text{cls}}^{\ell-1}, \mathbf{z}_{p}^{\ell-1}]) \quad \ell = 1, \dots, J-1
\end{align*}
For subsequent layers $\ell \ge J$, the process involves the attribute tokens. Let $\mathbf{r}_{\text{attr}}^{\ell-1}$ be the state of an attribute token before entering layer $\ell$. The Transformer layer $\mathcal{V}_{\ell}$ processes the augmented sequence to produce an updated, context-aware state $\tilde{\mathbf{r}}_{\text{attr}}^{\ell}$. The input to the \textit{next} layer, $\mathbf{r}_{\text{attr}}^{\ell}$, is then determined by a controlled mixture:
% \begin{align}
%     [\mathbf{z}_{\text{cls}}^{\ell}, \mathbf{z}_{p}^{\ell}, \{\tilde{\mathbf{r}}_{\text{attr}}^{\ell}\}_{\text{attr} \in A}] 
%     &= \mathcal{V}_{\ell}([\mathbf{z}_{\text{cls}}^{\ell-1}, \mathbf{z}_{p}^{\ell-1}, \{\mathbf{r}_{\text{attr}}^{\ell-1}\}_{\text{attr} \in A}]) \\[0.5em]
%     [\mathbf{z}_{\text{cls}}^{\ell+1}, \mathbf{z}_{p}^{\ell+1}, \{\tilde{\mathbf{r}}_{\text{attr}}^{\ell+1}\}_{\text{attr} \in A}] 
%     &= \mathcal{V}_{\ell+1}([\mathbf{z}_{\text{cls}}^{\ell}, \mathbf{z}_{p}^{\ell}, \nonumber \\
%     &\quad\quad \{\beta \cdot\mathbf{r}_{\text{attr}}^{\ell}+ (1 - \beta) \cdot \tilde{\mathbf{r}}_{\text{attr}}^{\ell}\}_{\text{attr} \in A}])\label{eq:knowledge_anchoring_vision}
% \end{align}
\begin{align}
&[\mathbf{z}_{\text{cls}}^{\ell}, \mathbf{z}_{p}^{\ell}, \{\tilde{\mathbf{r}}_{\text{attr}}^{\ell}\}_{\text{attr} \in A}] 
= \mathcal{V}_{\ell}([\mathbf{z}_{\text{cls}}^{\ell-1}, \mathbf{z}_{p}^{\ell-1}, \{\mathbf{r}_{\text{attr}}^{\ell-1}\}_{\text{attr} \in A}]) \nonumber \\
&[\mathbf{z}_{\text{cls}}^{\ell+1}, \mathbf{z}_{p}^{\ell+1}, \{\tilde{\mathbf{r}}_{\text{attr}}^{\ell+1}\}_{\text{attr} \in A}] \nonumber \\
&\quad = \mathcal{V}_{\ell+1}([\mathbf{z}_{\text{cls}}^{\ell}, \mathbf{z}_{p}^{\ell}, \{\beta \mathbf{r}_{\text{attr}}^{\ell}+ (1 - \beta) \tilde{\mathbf{r}}_{\text{attr}}^{\ell}\}_{\text{attr} \in A}])
\label{eq:knowledge_anchoring_vision}
\end{align}
Inspired by MMRL++ \citep{guo2025mmrlparameterefficientinteractionawarerepresentation}, we control the information flow between layers using the hyperparameter $\beta \in [0, 1]$. A purely sequential evolution ($\beta=0$) allows tokens to adapt fully to the context of vision feature, but risks "semantic drift," where the token deviates from its core learned meaning. Conversely, a static re-injection of the raw token at each layer ($\beta=1$) strongly preserves the core meaning but prevents any contextual adaptation. Our approach Eq. (\ref{eq:knowledge_anchoring_vision}) strikes a flexible balance: it allows the attribute token to absorb image-specific information via $\tilde{\mathbf{r}}_{\text{attr}}^{\ell}$ while being regularized by its foundational prior $\mathbf{r}_{\text{attr}}$. This prevents the representation from deviating excessively from its core attribute meaning, leading to more stable prompt learning.

\paragraph{Text-Side Prompting.}
To ensure cross-modal alignment, we apply a symmetrical strategy to the text encoder $\mathcal{W}$. We initialize a set of $K$ learnable tokens, $\{\mathbf{p}_k\}$, which are injected from layer $J$ to $L$ between the [BOT] and word tokens. Since text prompts for classification are typically simple templates (e.g., ``a photo of \{cls\}''), a small set of parameters suffices for alignment without needing attribute-specific designs. The forward pass through the text encoder is then modified. For any given layer $\ell$, let the full sequence of input tokens be $\mathbf{T}^{\ell-1}$. The output is computed as $\mathbf{T}^{\ell} = \mathcal{W}_{\ell}(\mathbf{T}^{\ell-1})$, where the prompt tokens within $\mathbf{T}^{\ell-1}$ are defined conditionally:
\begin{equation}
\label{eq:knowledge_anchoring_text}
\mathbf{p}_k^{\text{in}, \ell} = 
\begin{cases} 
    \mathbf{p}_k^{\ell-1} & \text{if } \ell < J \\
    \beta \mathbf{p}_k + (1-\beta) \tilde{\mathbf{p}}_k^{\ell-1} & \text{if } \ell \ge J
\end{cases}
\end{equation}
Here, $\mathbf{p}_k^{\text{in}, \ell}$ is the input prompt for layer $\ell$, $\tilde{\mathbf{p}}_k^{\ell-1}$ is the context-aware output from the previous layer, and $\mathbf{p}_k$ is the initial raw token. This controlled mixture, governed by $\beta$, allows contextual adaptation while preventing semantic drift. At inference, only the final [EOT] feature is used.
% \paragraph{Text-Side Prompting.}

% To ensure cross-modal alignment, we apply a symmetrical strategy to the text encoder $\mathcal{W}$. We initialize a set of $K$ learnable tokens, $\{\mathbf{p}_k \in \mathbb{R}^{D_t}\}_{k=1}^K$, where $D_t$ is the dimension of the text feature. These tokens are injected into the text encoder also from layer $J$ to $L$. The text prompts are inserted between the [BOT] token and the word tokens. The same hyperparameter $\beta$ as introduced in the vision side is used to control the evolution of these text prompts. In classification task, the text encoder mainly provides anchor representations for matching with visual features. Since our prompts are usually simple templates like ``a photo of \{cls\}'', which contain limited information, we find that a small set of learnable parameters is sufficient for cross-modal alignment, without extra attribute-based designs. At inference, we use only the final EOT feature as the text representation.


% \begin{align*}
%     [\mathbf{t}_{\text{bot}}^{\ell}, \mathbf{t}_{\text{words}}^{\ell}, \mathbf{t}_{\text{eot}}^{\ell}] &= W_{\ell}([\mathbf{t}_{\text{bot}}^{\ell-1}, \mathbf{t}_{\text{words}}^{\ell-1}, \mathbf{t}_{\text{eot}}^{\ell-1}]) \quad \ell = 1, \dots, J-1
% \end{align*}
% For subsequent layers $\ell = J, \dots, L$. Let $\mathbf{p}_k^{\ell-1}$ be the state of a text prompt token entering layer $\ell$, and $\tilde{\mathbf{p}}_k^{\ell}$ be its context-aware state after processing by $\mathcal{W}_{\ell}$. The input to the next layer is then a controlled mixture of the context-aware state and the original raw prompt:

% \begin{align}
% &[\mathbf{t}_{\text{bot}}^{\ell}, \{\tilde{\mathbf{p}}_k^{\ell}\}_{k=1}^K, \mathbf{t}_{\text{words}}^{\ell}, \mathbf{t}_{\text{eot}}^{\ell}] \nonumber \\
% &\quad = \mathcal{W}_{\ell}([\mathbf{t}_{\text{bot}}^{\ell-1}, \{{\mathbf{p}}_k^{\ell-1}\}_{k=1}^K, \mathbf{t}_{\text{words}}^{\ell-1}, \mathbf{t}_{\text{eot}}^{\ell-1}]) \\
% &[\mathbf{t}_{\text{bot}}^{\ell+1}, \{\tilde{\mathbf{p}}_k^{\ell+1}\}_{k=1}^K, \mathbf{t}_{\text{words}}^{\ell+1}, \mathbf{t}_{\text{eot}}^{\ell+1}] \nonumber \\
% &\quad = \mathcal{W}_{\ell+1}([\mathbf{t}_{\text{bot}}^{\ell}, \{\beta \mathbf{p}_k^{\ell} + (1-\beta) \tilde{\mathbf{p}}_k^{\ell}\}_{k=1}^K, \mathbf{t}_{\text{words}}^{\ell}, \mathbf{t}_{\text{eot}}^{\ell}])
% \label{eq:knowledge_anchoring_text}
% \end{align}

% \begin{align}
% &[\mathbf{t}_{\text{bot}}^{\ell}, \{\tilde{\mathbf{p}}_k^{\ell}\}_{k=1}^K, \mathbf{t}_{\text{words}}^{\ell}, \mathbf{t}_{\text{eot}}^{\ell}] \nonumber \\
% &\quad = \mathcal{W}_{\ell}([\mathbf{t}_{\text{bot}}^{\ell-1}, \{{\mathbf{p}}_k^{\ell-1}\}_{k=1}^K, \mathbf{t}_{\text{words}}^{\ell-1}, \mathbf{t}_{\text{eot}}^{\ell-1}]) \nonumber \\
% &[\mathbf{t}_{\text{bot}}^{\ell+1}, \{\tilde{\mathbf{p}}_k^{\ell+1}\}_{k=1}^K, \mathbf{t}_{\text{words}}^{\ell+1}, \mathbf{t}_{\text{eot}}^{\ell+1}] \nonumber \\
% &\quad = \mathcal{W}_{\ell+1}([\mathbf{t}_{\text{bot}}^{\ell}, \{(1 - \beta) \mathbf{p}_k^{\ell} + \beta \tilde{\mathbf{p}}_k^{\ell}\}_{k=1}^K, \mathbf{t}_{\text{words}}^{\ell}, \mathbf{t}_{\text{eot}}^{\ell}])
% \label{eq:knowledge_anchoring_text}
% \end{align}

% This symmetrical setting allows the model to co-adapt representations, facilitating alignment between newly acquired visual attribute knowledge and the textual descriptions.
\begin{figure}[t!] % 使用figure*环境使其跨双栏，[t!]使其尽量置于页面顶部
    \centering % 图片居中
    \includegraphics[width=0.5\textwidth]{author-kit-CVPR2026-v1-latex-/img/token_cropped.pdf} % 关键命令
    \caption{
        Results of attribute-conditioned image retrieval on ImageNet. For each query image, we retrieval using features from different learned attribute tokens.
    }
    \label{fig:retrieval_analysis} % 用于在正文中引用图片的标签
\end{figure}

\subsubsection{Role-Based Attention Mask}
\label{sec:role_based_mask} % Changed label for better referencing

Preserving generalization requires precise control over the information flow between the original and newly introduced attribute tokens. Building on our data-driven identification of head roles, we introduce a \textbf{role-based attention mask} mechanism. This mechanism, applied within the deeper layers of the ViT ($l \ge J$), assigns a custom attention mask $\mathbf{M}_{(l,h)} \in \{-\infty, 0\}^{N_{seq} \times N_{seq}}$ to each head $(l,h)$ based on its specific function. The mask is applied additively to the raw attention scores:
\begin{equation}
\mathbf{S}_{(l,h)} = \frac{\mathbf{Q}_{(l,h)}\mathbf{K}_{(l,h)}^T}{\sqrt{D_h}} + \mathbf{M}_{(l,h)}
\label{eq:masked_scores}
\end{equation}
An entry $\mathbf{M}_{(l,h)}[i, j] = -\infty$ effectively severs the connection from query token $i$ to key token $j$ by setting its corresponding attention weight to zero post-softmax.

To formally define the masks, we partition the token indices into disjoint sets: $\mathcal{I}_{\text{cls}}$ for the \texttt{[CLS]} token, $\mathcal{I}_{\text{patch}}$ for patch tokens, and $\mathcal{I}_{\text{attr}}$ for our learnable attribute tokens. The set of original token indices is $\mathcal{I}_{\text{orig}} = \mathcal{I}_{\text{cls}} \cup \mathcal{I}_{\text{patch}}$. The mask construction depends on the head's role:

\paragraph{Generalization and Other Specialized Heads.}
This category includes both \textbf{Generalization Heads}, and other \textbf{Specialized Heads} not selected as core attributes (e.g., for 'numbers' or 'text'). We hypothesize that both types of heads encode the model's intrinsic, pre-trained capabilities that are crucial for zero-shot generalization. To protect these foundational abilities from being perturbed by task-specific information, we implement a strict mask. This mask prohibits any interaction between the original tokens and our five learnable attribute tokens:
\begin{equation}
\mathbf{M}_{(l,h)}[i, j] = 
\begin{cases} 
-\infty & \text{if } (i \in \mathcal{I}_{\text{orig}} \text{ and } j \in \mathcal{I}_{\text{attr}}) \\
& \text{or } (i \in \mathcal{I}_{\text{attr}} \text{ and } j \in \mathcal{I}_{\text{orig}}) \\
0 & \text{otherwise}
\end{cases}
\end{equation}
This policy ensures that both generalist heads and other specialist heads remain isolated, preserving their original functions.

\paragraph{Core Attribute Heads.}
These are the heads identified as specializing in one of our five core visual attributes $a \in A$ (\textit{e.g., 'color'}). The mask for such a head is designed to channel the corresponding learnable attribute token exclusively to its expert head, enabling focused learning. Let $\mathcal{I}_{\text{attr}(a)} \subset \mathcal{I}_{\text{attr}}$ be the index set for the token(s) corresponding to attribute $a$. The mask is defined as:
\begin{equation}
\mathbf{M}_{(l,h)}[i, j] = 
\begin{cases} 
-\infty & \text{if } j \in \mathcal{I}_{\text{attr}} \text{ and } j \notin \mathcal{I}_{\text{attr}(a)} \\
0 & \text{otherwise}
\end{cases}
\end{equation}
This rule allows any query token to attend to all original tokens and its relevant attribute token, while blocking attention to irrelevant ones. This promotes clean, disentangled attribute learning.

\paragraph{Mixed Heads.}
Heads with intermediate Concept Entropy are classified as \textbf{Mixed Heads}. We consider their function to be multifaceted and flexible. Therefore, we permit unrestricted attention by applying an all-zeros mask where $\mathbf{M}_{(l,h)}[i, j] = 0, \forall i, j$, allowing them to integrate information freely from all available tokens.
% \subsubsection{Role-Based Attention Mask}
% The key to preserving generalization lies in precisely controlling the interaction between original tokens and new attribute tokens. We introduce a \textbf{role-based attention Mask} mechanism within the deeper layers of the ViT ($l \ge J$). For each head $(l,h)$, we apply a custom attention mask $\mathbf{M}_{(l,h)} \in \{-\infty, 0\}^{N_{seq} \times N_{seq}}$ based on its pre-identified functional role, where ${N_{seq}}$ denote that the number of all tokens, including the CLS token, patch tokens and attribute tokens. This mask is applied additively to the raw attention scores before the softmax normalization:
% \begin{equation}
% \mathbf{S}_{(l,h)} = \frac{\mathbf{Q}_{(l,h)}\mathbf{K}_{(l,h)}^T}{\sqrt{D_h}} + \mathbf{M}_{(l,h)}
% \label{eq:masked_scores}
% \end{equation}
% The attention weights are then derived as $\boldsymbol{\alpha}_{(l,h)} = \text{softmax}(\mathbf{S}_{(l,h)})$. If $\mathbf{M}_{(l,h)}[i, j] = -\infty$, the corresponding weight $\alpha_{(l,h)}^{i \to j}$ becomes zero, effectively severing the connection. The mask structure depends on the head's role. \textbf{For Generalization Heads:} A strict "information firewall" is erected, preventing original tokens from interacting with new attribute tokens. \textbf{For Attribute Heads:} A specialized mask is applied, restricting attention to only relevant attribute tokens. \textbf{For Mixed Heads:} An all-zeros mask is used ($\mathbf{M}_{(l,h)} = \mathbf{0}$), permitting unrestricted attention.This per-head control of information flow is the core mechanism allowing A-Prompt to learn fine-grained attributes while preserving generalization.

\subsubsection{Final Feature Generation.}
After passing through all $L$ layers, the final hidden states of the \texttt{[CLS]} and attribute tokens are projected to generate features. The state of the original class token, $\mathbf{z}_{\text{cls}}^L$, is projected by the pre-trained and \textbf{frozen} vision projection head, $\mathbf{P}_{\text{vision}}(\cdot)$, to yield the class feature $\mathbf{f}_{\text{cls}}$:
\begin{equation}
    \label{eq:fc_generation}
    \mathbf{f}_{\text{cls}} = \mathbf{P}_{\text{vision}}(\text{LN}(\mathbf{z}_{\text{cls}}^L))
\end{equation}
Similarly, the final state of each attribute token, $\mathbf{r}_{\text{attr}}^L$, is processed by a shared, \textbf{trainable} projection head, $\mathbf{P}_{\text{attr}}(\cdot)$, to yield a set of specialized attribute features $\{\mathbf{f}_{\text{attr}}\}$:
\begin{equation}
    \label{eq:fr_generation}
    \mathbf{f}_{\text{attr}} = \mathbf{P}_{\text{attr}}(\text{LN}(\mathbf{r}_{\text{attr}}^L))
\end{equation}
This process yields a primary feature $\mathbf{f}_cls$ retaining generalization, and specialized features $\mathbf{f}_\text{attr}$.




% $\{\mathbf{f}_{\text{color}}, \mathbf{f}_{\text{shape}}, \mathbf{f}_{\text{object}}, \mathbf{f}_{\text{texture}}, \mathbf{f}_{\text{location}}\}$
% encoding fine-grained knowledge.




To visually validate our attribute tokens capture semantic concepts, we conduct an attribute-conditioned image retrieval, shown in Figure~\ref{fig:retrieval_analysis}. 

% We use the final attribute features from a query image to search for similar images in the ImageNet dataset. The results are striking. For the penguin input, the \textbf{object token} correctly retrieves other penguins, while the \textbf{color token} retrieves unrelated black-and-white items like a piano and a Dalmatian dog. This pattern is mirrored for the pyramid query: the \textbf{location token} retrieves similar scenes, while the \textbf{texture token} finds images of sand.

% \subsubsection{Training and Inference}
% \label{sec:training_inference}

% \paragraph{Training.}
% The A-Prompt training process is designed to optimize both the classification accuracy and the preservation of generalization. The final loss function is a weighted sum of a primary classification loss and several regularization terms. The primary classification loss is the standard cross-entropy loss, $\mathcal{L}_{\text{CE}}(\hat{\mathbf{y}}, \mathbf{y})$, where $\hat{\mathbf{y}}$ are the predicted logits from our fusion strategy (defined in Eq.~\ref{eq:fusion_explicit}).

% To preserve the model's foundational generalization, we introduce a self-regularization loss, $\mathcal{L}_{\text{reg}}$. This term encourages the final features from both the vision and text encoders to remain close to their original, unmodified CLIP. Specifically, we regularize both the final class feature $\mathbf{f}_cls$ and the text feature $\mathbf{f}_t$:
% \begin{align}
%     \mathcal{L}_{\text{reg}}^V &= 1 - \text{cos}(\mathbf{f}_c, \mathbf{f}_{c}^{\text{orig}}) \\
%     \mathcal{L}_{\text{reg}}^T &= 1 - \text{cos}(\mathbf{f}_t, \mathbf{f}_{t}^{\text{orig}}) \\
%     \mathcal{L}_{\text{reg}} &= \mathcal{L}_{\text{reg}}^V + \mathcal{L}_{\text{reg}}^T
% \end{align}


% where $\mathbf{f}_{c}^{\text{orig}}$ and $\mathbf{f}_{t}^{\text{orig}}$ are the corresponding features from the frozen, original CLIP model.

% Furthermore, to ensure the model does not over-rely on the learned attribute features, a fusion-weight regularization, $\mathcal{L}_{\text{fusion}}$, encourages the fusion mechanism to prioritize the class feature:
% \begin{equation}
%     \mathcal{L}_{\text{fusion}} = -\log(\alpha_\text{cls})
% \end{equation}
% where $\alpha_\text{cls}$ is the softmax-normalized weight from Eq.~\eqref{eq:softmax_weights}. The total training loss is a weighted combination of these objectives:
% \begin{equation}
%     \mathcal{L}_{\text{total}} = \mathcal{L}_{\text{CE}} + \lambda_{\text{reg}} \mathcal{L}_{\text{reg}} + \lambda_{\text{fusion}} \mathcal{L}_{\text{fusion}}
% \end{equation}
% where $\lambda_{\text{reg}}$ and $\lambda_{\text{fusion}}$ are balancing hyperparameters.

% \paragraph{Task-Adaptive Fusion for Inference.}
% We propose a Task-Adaptive Fusion strategy for inference. We learn a small set of fusion weights, $\{w_k\}_{k \in \{\text{cls}\} \cup A}$, on the base classes, which are then fixed and used for novel classes. For a given image and a set of $m$ class text embeddings $\{\mathbf{t}_j\}_{j=1}^m$, we first compute similarity vectors for the class feature $\mathbf{f}_cls$ and each attribute feature $\mathbf{f}_\text{attr}$:
% \begin{align}
%     \mathbf{s}_c &= \tau \cdot [\text{sim}(\mathbf{f}_{c}, \mathbf{t}_1), \dots, \text{sim}(\mathbf{f}_{c}, \mathbf{t}_m)] \\
%     \mathbf{s}_{\text{attr}} &= \tau \cdot [\text{sim}(\mathbf{f}_{\text{attr}}, \mathbf{t}_1), \dots, \text{sim}(\mathbf{f}_{\text{attr}}, \mathbf{t}_m)]
% \end{align}
% where $\tau$ is CLIP's trainable temperature parameter. The final logits $\hat{\mathbf{y}}$ are a weighted sum of these similarity vectors, with weights derived via softmax to ensure they sum to 1:
% \begin{equation}
% \label{eq:fusion_explicit}
%     \hat{\mathbf{y}} = \alpha_c \cdot \mathbf{s}_c + \sum_{\text{attr} \in A} \alpha_\text{attr} \cdot \mathbf{s}_\text{attr}
% \end{equation}
% where the fusion weights $\alpha_k$ are calculated as:
% \begin{equation}
% \label{eq:softmax_weights}
%     \alpha_k = \frac{e^{w_k}}{e^{w_c} + \sum_{i \in A} e^{w_i}}, \quad \text{for } k \in \{c\} \cup A
% \end{equation}
% We propose the task-adaptive inference strategy based on the suppose that, for the same downstream task, the model's reliance on attribute information during inference should follow a consistent pattern. This approach enables the model to capture task-level priors (e.g., bird classification often depends on color cues) and apply them to unseen classes, resulting in a more principled and effective fusion mechanism.


\subsubsection{Training and Inference}
\label{sec:training_inference}

\paragraph{Training.}
DeAR's training process balances classification accuracy on the target task with preserving the model's pre-trained generalization. The total loss function is a weighted combination of a primary classification loss and two regularization terms:
\begin{equation}
    \mathcal{L}_{\text{total}} = \mathcal{L}_{\text{CE}} + \lambda_{\text{reg}} \mathcal{L}_{\text{reg}} + \lambda_{\text{fusion}} \mathcal{L}_{\text{fusion}}
\label{eq:total_loss}
\end{equation}
where $\lambda_{\text{reg}}$ and $\lambda_{\text{fusion}}$ are hyperparameters that balance the contribution of each component.

The primary loss, $\mathcal{L}_{\text{CE}}(\hat{\mathbf{y}}, \mathbf{y})$, is the standard cross-entropy between the predicted logits $\hat{\mathbf{y}}$ (defined in our inference strategy \citep{mao2023crossentropylossfunctionstheoretical}, Eq.~\ref{eq:fusion_explicit}) and the ground-truth labels $\mathbf{y}$.

To preserve the model's foundational knowledge, we introduce a self-regularization loss, $\mathcal{L}_{\text{reg}}$. This term encourages the final features from both the vision and text encoders to remain close to their counterparts from the original, frozen CLIP model. Specifically, we regularize the final class feature $\mathbf{f}_{\text{cls}}$ and the text feature $\mathbf{f}_t$:
\begin{align}
    \mathcal{L}_{\text{reg}} &= \mathcal{L}_{\text{reg}}^V + \mathcal{L}_{\text{reg}}^T \\
    \quad \mathcal{L}_{\text{reg}}^V &= 1 - \text{cos}(\mathbf{f}_{\text{cls}}, \mathbf{f}_{\text{cls}}^{\text{orig}}) \\
    \quad \mathcal{L}_{\text{reg}}^T &= 1 - \text{cos}(\mathbf{f}_t, \mathbf{f}_{t}^{\text{orig}})
\end{align}
Here, $\mathbf{f}_{\text{cls}}^{\text{orig}}$ and $\mathbf{f}_{t}^{\text{orig}}$ are the features extracted from the unmodified CLIP model, and $\text{cos}(\cdot, \cdot)$ denotes the cosine similarity.

To prevent over-reliance on the newly learned attribute features, we introduce a fusion-weight regularization, $\mathcal{L}_{\text{fusion}}$. This loss encourages the inference mechanism to assign a higher weight to the more general class feature:
\begin{equation}
    \mathcal{L}_{\text{fusion}} = -\log(\alpha_{\text{cls}})
\end{equation}
where $\alpha_{\text{cls}}$ is the softmax-normalized weight corresponding to the class feature.


\paragraph{Task-Adaptive Fusion for Inference.}
For inference, we propose a \textbf{Task-Adaptive Fusion} strategy that combines evidence from the protected class and specialized attribute features. We learn a small set of scalar weights, $\{w_k\}_{k \in \{\text{cls}\} \cup A}$, on the base classes, which are then fixed for novel classes.

For a given image and $m$ class text embeddings $\{\mathbf{t}_j\}_{j=1}^m$, we first compute similarity vectors for the class feature $\mathbf{f}_{\text{cls}}$ and each attribute feature $\mathbf{f}_{a}$:
\begin{align}
    \mathbf{s}_{\text{cls}} &= \tau \cdot [\text{sim}(\mathbf{f}_{\text{cls}}, \mathbf{t}_1), \dots, \text{sim}(\mathbf{f}_{\text{cls}}, \mathbf{t}_m)] \\
    \mathbf{s}_{a} &= \tau \cdot [\text{sim}(\mathbf{f}_{a}, \mathbf{t}_1), \dots, \text{sim}(\mathbf{f}_{a}, \mathbf{t}_m)]
\end{align}
where $\tau$ is CLIP's frozen temperature parameter. The final logits $\hat{\mathbf{y}}$ are a weighted sum of these vectors. The fusion weights $\alpha_k$ are derived from the learned scalars $\{w_k\}$ via softmax, where $\alpha_k = e^{w_k} / (e^{w_{\text{cls}}} + \sum_{i \in A} e^{w_i})$. The final logits are then computed as:
\begin{equation}
    \hat{\mathbf{y}} = \alpha_{\text{cls}} \cdot \mathbf{s}_{\text{cls}} + \sum_{a \in A} \alpha_a \cdot \mathbf{s}_a.
    \label{eq:fusion_explicit}
\end{equation}
This strategy assumes that a model's reliance on specific attributes is a task-level prior (e.g., color is important for bird classification). By learning and transferring these priors, we achieve a more principled and effective fusion.


% The heatmap Figure~\ref{fig:heat_map} illustrates how A-Prompt learns to rely on different features for different tasks. For instance, the model assigns the higher weight to the Texture feature on the DTD dataset and to the Shape feature on FGVCAircraft, validating our hypothesis that the fusion mechanism captures task-level priors.

% \begin{figure}[t!] % 使用figure*环境使其跨双栏，[t!]使其尽量置于页面顶部
%     \centering % 图片居中
%     \includegraphics[width=0.5\textwidth]{author-kit-CVPR2026-v1-latex-/sec/fusion_weights_academic_final_cropped (1).pdf} % 关键命令
%     \caption{
%         Visualization of learned Task-Adaptive Fusion weights $\alpha_k$ across 11 datasets.
%     }
%     \label{fig:heat_map} % 用于在正文中引用图片的标签
% \end{figure}

==> sec/4_experiment.tex <==
\section{Experiments}
% Detailed implementation, code, complete experiment results, hyperparameters settings and more ablation experiments are provided in the appendix.
\input{author-kit-CVPR2026-v1-latex-/sec/b2n}

% \subsection{Experiment Setting}
% \label{sec:exp_setup}

% To comprehensively evaluate the effectiveness and generalization capabilities of our proposed DeAR framework, we conduct four evaluations: (1) base-to-novel generalization, (2) domain generalization, (3) few-shot learning and (4) cross-dataset generalization. Except few-shot learning, all experiments are conducted in a 16-shot setting, where the model is trained on only 16 labeled examples per category.
\subsection{Experiment settings}
\paragraph{Implementation Details.}
Our implementation is based on the OpenCLIP with a ViT-B-16 backbone. We train the model using the AdamW optimizer with an initial learning rate of $1 \times 10^{-3}$. All experiments are conducted on three NVIDIA RTX 4090 GPUs. Further details are provided in the Appendix.
\paragraph{Base-to-Novel Generalization.}
% \subsection{Base-to-Novel Generalization}
This is the primary evaluation to assess DeAR's ability to adapt to downstream tasks while preserving generalization. We conduct this evaluation across eleven image classification datasets: ImageNet \citep{5206848}, Caltech101 \citep{1384978}, OxfordPets \citep{6248092}, StanfordCars \citep{6755945}, Flowers102 \citep{4756141}, Food101 \citep{10.1007/978-3-319-10599-4_29}, FGVCAircraft \citep{maji2013finegrainedvisualclassificationaircraft}, SUN397 \citep{5539970}, UCF101 \citep{Soomro2012UCF101AD}, DTD \citep{6909856}, and EuroSAT \citep{8736785}. We follow the standard setup: the model trains on 16-shot base classes and is evaluated on the test sets of both base and novel classes. As shown in Table~\ref{b2n}, DeAR demonstrates clear superiority, achieving a new state-of-the-art harmonic mean of 82.72\%. This result is driven by a significant 1.83\% improvement on novel classes over the previous best, MMRL. The substantial gain on unseen classes directly validates our core hypothesis: protecting generalization heads is crucial for preserving the model's foundational knowledge.

\paragraph{Domain Generalization.}
% \subsection{Domain Generalization}
This evaluation measures the model's robustness to out-of-distribution data and domain shifts. Following standard practice, we train the model on the 16-shot ImageNet training set (all classes) and directly evaluate its performance, without further fine-tuning, on four challenging ImageNet variants: ImageNetV2 \citep{Recht2019DoIC}, ImageNet-Sketch \citep{NEURIPS2019_3eefceb8}, ImageNet-A \citep{9578772}, and ImageNet-R \citep{9710159}. Table~\ref{tab:domain_gen_results} presents the domain generalization results. Our method demonstrates consistently strong robustness across all four out-of-distribution datasets. DeAR achieves the best performance on ImageNet-A (51.80\%) and ImageNet-R (78.83\%), also is highly competitive in the other variants.
\input{author-kit-CVPR2026-v1-latex-/sec/cross_dataset}
\input{author-kit-CVPR2026-v1-latex-/sec/generalization}
% \subsection{Few-Shot Learning}
\paragraph{Few-Shot Learning.}
Few-shot learning evaluates the capacity of the model for knowledge transfer and generalization when labeled data are limited. To quantify this capability, we fine-tune DeAR on $k$ shot subsets of the original training data, where $k\in\{1,2,4,8,16\}$. As shown in Figure~\ref{fig:few_shot}, across all settings from 1 to 16 shots, DeAR consistently outperforms the baseline methods, demonstrating a slight but consistent performance advantage. This suggests that our DeAR framework provides robust performance even in limited labeled data. Detailed results on all 11 datasets are provided in the Appendix. 

% \subsection{Cross-Dataset Generalization}
\paragraph{Cross-Dataset Generalization.}
To evaluate transfer ability, we train DeAR on ImageNet (16 shots per class) and test it zero-shot on ten unseen datasets. Since the Task-Adaptive Fusion weights are optimized for ImageNet, they may not generalize. Therefore, for a fair evaluation on the target datasets, we adopt a decoupled inference strategy similar to MMRL~\citep{guo2025mmrl}, using only the protected class feature $\mathbf{f}_{\text{cls}}$ for prediction. As shown in Table~\ref{tab:cross_dataset_results}, DeAR sets a new state-of-the-art average accuracy of 67.60\%, surpassing the previous best method, MMRL, while maintaining comparable performance on the source task (ImageNet).
% its enhanced transferability to unseen datasets highlights the critical importance of role-based attention mask mechnism.




\begin{figure}[htbp]
     \centering
     \includegraphics[width=0.4\textwidth]{author-kit-CVPR2026-v1-latex-/sec/figure_high_resolution.pdf}%
    \caption{Comparison of DeAR with previous methods on few-shot learning. Detailed results are provided in the Appendix}
    \label{fig:few_shot}
\end{figure}



% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.23\textwidth]{AuthorKit26/AnonymousSubmission/LaTeX/few_shot.pdf}%
% %     \hspace{0.01\textwidth}%
%     \includegraphics[width=0.23\textwidth]{AuthorKit26/AnonymousSubmission/LaTeX/fewshot2.pdf}
%     % \caption{Comparison of DeAR with previous methods on few-shot learning. Detailed results are provided in the Appendix}
%     \caption{Comparison of DeAR with previous methods on few-shot learning.}
%     \label{fig:few_shot}
% \end{figure}



\subsection{Ablation Studies}
To validate the effectiveness of the key components in our DeAR framework, we conduct a series of ablation studies on the average performance across all 11 datasets in the base-to-novel generalization setting.

\paragraph{Role-Based Attention Mask.}
To validate our core hypothesis, that role-based information control is superior to uniform strategies, we compare DeAR against two variants: All-Generalization, where all deep heads are shielded from attribute tokens, and All-Mixed, where all interactions are permitted.
% \begin{itemize}
%     \item \textbf{All-Generalization:} All attention heads in the deep layers ($l \ge J$) are treated as Generalization Heads, applying the restrictive mask that blocks all interaction with attribute tokens.
%     \item \textbf{All-Mixed:} All deep attention heads are treated as Mixed Heads, permitting unrestricted interaction between original and attribute tokens.
% \end{itemize}

% \begin{table}[h!]
% \centering
% \caption{Ablation study on the Role-Based Attention Mask mechanism.}
% \label{tab:ablation_Mask}
% \resizebox{0.4\textwidth}{!}{
% \begin{tabular}{lccc}
% \toprule
% \textbf{Mask Strategy} & \textbf{Base} & \textbf{Novel} & \textbf{HM} \\
% \midrule
% All-Generalization & 81.25 & \textbf{80.12} & 80.68 \\
% All-Mixed & 85.31 & 76.98 & 80.93 \\
% \midrule
% \textbf{DeAR (Ours)} & \textbf{85.94} & 79.73 & \textbf{82.72} \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

The results shown in Table~\ref{tab:ablation_Mask} validate our role-based design. The All-Generalization strategy maximizes novel-class performance at the cost of base-class learning, while the All-Mixed strategy does the opposite. Our proposed DeAR strikes the optimal balance between adaptation and generalization, achieving the best overall Harmonic Mean.

\begin{table}[h!]
\centering
\caption{Ablation on Role-Based Attention Mask.}
\small % 或者 \footnotesize, \scriptsize
\begin{tabular}{lccc}
    \toprule
    Mask Strategy & Base & Novel & HM \\
    \midrule
    All-Generalization & 81.25 & \textbf{80.12} & 80.68 \\
    All-Mixed & 85.31 & 76.98 & 80.93 \\
    \rowcolor{gray!20} % 为您方法所在行添加背景色
    \textbf{DeAR (Ours)} & \textbf{85.94} & 79.73 & \textbf{82.72} \\
    \bottomrule
\end{tabular}
\label{tab:ablation_Mask}
\end{table}

\paragraph{Impact of Loss Components.}
We also analyze the contribution of each component in our proposed loss function. We start with a baseline using only the cross-entropy classification loss ($\mathcal{L}_{\text{CE}}$) and incrementally add our two regularization terms: the multimodal self-regularization ($\mathcal{L}_{\text{reg}}$) and the fusion-weight regularization ($\mathcal{L}_{\text{fusion}}$).

% \begin{table}[h!]
% \centering
% \caption{Ablation study on the components of the loss function.}
% \label{tab:ablation_loss}
% \resizebox{0.4\textwidth}{!}{
% \begin{tabular}{lccc}
% \toprule
% \textbf{Loss Function} & \textbf{Base} & \textbf{Novel} & \textbf{HM} \\
% \midrule
% $\mathcal{L}_{\text{CE}}$ & \textbf{86.75} & 74.21 & 79.99 \\
% $\mathcal{L}_{\text{CE}}$ + $\mathcal{L}_{\text{reg}}$ & 85.03 & 78.45 & 81.61 \\
% \midrule
% $\mathcal{L}_{\text{CE}}$ + $\mathcal{L}_{\text{reg}}$ + $\mathcal{L}_{\text{fusion}}$  & 85.94 & \textbf{79.73} & \textbf{82.72} \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

As shown in Table~\ref{tab:ablation_loss}, each loss component is vital. Adding $\mathcal{L}_{\text{reg}}$ significantly boosts Novel class performance (+4.24\%). The subsequent addition of $\mathcal{L}_{\text{fusion}}$ further improves the overall Harmonic Mean, demonstrating the benefit of prioritizing the class feature.




\begin{table}[h!]
\centering
\caption{Ablation on Loss function components.}
\small % 或者 \footnotesize, \scriptsize
\begin{tabular}{lccc}
    \toprule
    Loss Function & Base & Novel & HM \\
    \midrule
    $\mathcal{L}_{\text{CE}}$ & \textbf{86.75} & 74.21 & 79.99 \\
    $\mathcal{L}_{\text{CE}}$ + $\mathcal{L}_{\text{reg}}$ & 85.03 & 78.45 & 81.61 \\
    \rowcolor{gray!20} % 为您方法所在行添加背景色
    $\mathcal{L}_{\text{CE}}$ + $\mathcal{L}_{\text{reg}}$ + $\mathcal{L}_{\text{fusion}}$ & 85.94 & \textbf{79.73} & \textbf{82.72} \\
    \bottomrule
\end{tabular}
\label{tab:ablation_loss}
\end{table}

% \paragraph{Baselines.}
% We compare DeAR against several state-of-the-art prompt learning methods to demonstrate its superiority. These include the pioneering text-prompting method CoOp \citep{Zhou_2022} and its instance-conditioned successor CoCoOp \citep{zhou2022cocoop}. We also benchmark against the first multimodal prompting method, MaPLe \citep{khattakMaPLe}, and its advanced follow-up, MMRL \citep{guo2025mmrl}, which represents the current state-of-the-art and shares our focus on deep-layer prompting. For reference, we also report the performance of the original zero-shot CLIP model as a fundamental baseline.

% \paragraph{Implementation Details.}
% Our implementation is based on PyTorch. We use the pre-trained ViT-B-16 as the vision encoder and the corresponding Transformer as the text encoder from the official CLIP release. 
% \begin{itemize}
%     \item \textbf{DeAR Setup:} Based on our analysis, we initialize 5 attribute tokens for the vision side ($A = \{\text{color, shape, texture, object, location}\}$). We also use $K=4$ general-purpose prompt tokens for the text side. All learnable tokens are injected starting from layer $J=8$ in both encoders.
%     \item \textbf{Training:} We use the AdamW optimizer \citep{loshchilov2018decoupled} with a batch size of 32. The learning rate is set to $2 \times 10^{-4}$ for all newly introduced learnable parameters (attribute/prompt tokens, projection layers, and fusion weights), with a cosine annealing learning rate schedule. All models are trained for 10 epochs.
%     \item \textbf{Hyperparameters:} The knowledge anchoring weight $\beta$ is set to 0.5 based on validation experiments. The regularization hyperparameters for the loss function are set to $\lambda_{\text{reg}} = 0.1$ and $\lambda_{\text{fusion}} = 0.05$. All other hyperparameters follow those of the baseline methods for fair comparison.
% \end{itemize}
% All experiments are conducted on NVIDIA A100 GPUs.


==> sec/5_conclusion.tex <==
\section{Conclusion}


In this work, we propose the DeAR framework to enhance the adaptation of CLIP by balancing task-specific knowledge with generalization preservation. DeAR offers a fine-grained controllable fine-tuning process. Using our Concept Entropy, we decompose each attention head roles, allowing DeAR to direct new knowledge to attribute heads while protecting generalization heads. Experiments show that DeAR achieves state-of-the-art performance on base-to-novel generalization benchmarks and performs well on various tasks. More importantly, the learned attribute-aware representations offer significant potential for future applications requiring explicit semantic control, such as fine-grained retrieval. We demonstrate that fine-grained internal control is the path to better VLMs adaptation.

==> sec/b2n.tex <==
\begin{table*}[ht]
\centering
\caption{Comparison of DeAR with previous methods on base-to-novel generalization across 11 datasets. Bold values indicate the best results.}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Method} 
    & \multicolumn{3}{c|}{Average} 
    & \multicolumn{3}{c|}{ImageNet} 
    & \multicolumn{3}{c|}{Caltech101} 
    & \multicolumn{3}{c|}{OxfordPets}
    & \multicolumn{3}{c|}{StanfordCars} 
    & \multicolumn{3}{c}{Flowers102} \\
 & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM \\
\midrule
CLIP \scriptsize{(ICML2021)}          & 69.34 & 74.22 & 71.70 & 72.43 & 68.14 & 70.22 & 96.84 & 94.00 & 95.40 & 91.17 & 97.96 & 94.12 & 63.37 & 74.89 & 68.65 & 72.08 & 77.80 & 74.83 \\
CoOp \scriptsize{(ICCV2021)}          & 82.69 & 63.22 & 71.66 & 76.47 & 67.88 & 71.92 & 98.01 & 89.81 & 93.73 & 93.67 & 95.29 & 94.47 & 78.12 & 60.40 & 68.13 & 97.60 & 59.67 & 74.06 \\
ATPrompt$_{CoOp}$ \scriptsize{(ICCV2025)} & 82.68 & 68.04 & 74.65 & 76.27 & 70.60 & 73.33 & 97.95 & 93.63 & 95.74 & 94.77 & 96.59 & 95.67 & 77.43 & 66.55 & 71.58 & 97.44 & 67.52 & 79.77 \\
ProGrad \scriptsize{(CVPR2023)}         & 82.48 & 70.75 & 76.16 & 77.02 & 66.66 & 71.46 & 98.02 & 93.89 & 95.91 & 95.07 & 97.63 & 96.33 & 77.68 & 68.63 & 72.88 & 95.54 & 71.87 & 82.03 \\
MaPLe \scriptsize{(CVPR2023)}         & 82.28 & 75.14 & 78.55 & 76.60 & 70.54 & 73.47 & 97.74 & 94.36 & 96.02 & 95.43 & 97.76 & 96.58 & 72.94 & 74.00 & 73.47 & 95.92 & 72.46 & 82.56 \\
PromptSRC \scriptsize{(ICCV2023)}     & 84.26 & 76.10 & 79.97 & 77.60 & 70.73 & 74.01 & 98.10 & 94.03 & 96.02 & 95.33 & 97.30 & 96.30 & 78.27 & 74.97 & 76.58 & 98.07 & 76.50 & 85.95 \\
ProVP \scriptsize{(CVPR2024)}        & 85.20 & 73.22 & 78.76 & 75.82 & 69.21 & 72.36 & 98.92 & 94.21 & 96.51 & 95.87 & 97.65 & 96.75 & 80.43 & 67.96 & 73.67 & 98.42 & 72.06 & 83.20 \\
TCP \scriptsize{(CVPR2024)}           & 84.13 & 75.36 & 79.51 & 77.27 & 69.87 & 73.38 & 98.23 & 94.67 & 96.42 & 94.67 & 97.20 & 95.92 & 80.80 & 74.13 & 77.32 & 97.73 & 75.57 & 85.23 \\
PromptKD \scriptsize{(CVPR2024)}      & 84.11 & 78.28 & 81.09 & 77.63 & 70.96 & 74.15 & 98.31 & \textbf{96.29} & \textbf{97.29} & 93.42 & 97.44 & 95.39 & 80.48 & \textbf{81.78} & \textbf{81.12} & 98.69 & \textbf{81.91} & \textbf{89.52} \\
MMRL \scriptsize{(CVPR2025)}          & 85.68 & 77.16 & 81.20 & 77.90 & 71.30 & 74.45 & 98.97 & 94.50 & 96.68 & 95.90 & 97.60 & 96.74 & 81.30 & 75.07 & 78.06 & 98.97 & 77.27 & 86.78 \\
TAC \scriptsize{(CVPR2025)}           & 85.24 & 77.60 & 81.24 & \textbf{78.57} & 71.03 & 74.61 & 98.57 & 95.27 & 96.89 & 95.93 & \textbf{98.17} & \textbf{97.04} & 81.63 & 74.17 & 77.72 & 97.97 & 76.87 & 86.15 \\
SkipT \scriptsize{(CVPR2025)} & 85.04 & 77.53 & 81.11 & 77.73 & 70.40 & 73.89 & 98.50 & 95.33 & 96.89 & 95.70 & 97.87 & 96.77 & \textbf{82.93} & 72.50 & 77.37 & 98.57 & 75.80 & 85.70 \\
\midrule
\rowcolor{lightgray} 
\textbf{DeAR (Ours)}                   & \textbf{85.94} & \textbf{79.73} & \textbf{82.72} & 78.12 & \textbf{71.80} & \textbf{74.83} & \textbf{99.00} & 95.80 & 96.95 & \textbf{97.34} & 97.50 & 96.81 & 82.01 & 75.20 & 78.47 & \textbf{99.00} & 78.50 & 87.57 \\
\bottomrule
\end{tabular}
}
\vspace{0.1cm}

\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Method} 
    & \multicolumn{3}{c|}{Food101} 
    & \multicolumn{3}{c|}{FGVC Aircraft} 
    & \multicolumn{3}{c|}{SUN397} 
    & \multicolumn{3}{c|}{DTD}
    & \multicolumn{3}{c|}{EuroSAT}
    & \multicolumn{3}{c}{UCF101} \\
 & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM \\
\midrule
CLIP \scriptsize{(ICML2021)}          & 90.10 & 91.22 & 90.66 & 27.19 & 36.29 & 31.09 & 69.36 & 75.35 & 72.23 & 53.24 & 59.90 & 56.37 & 56.48 & 64.05 & 60.03 & 70.53 & 77.50 & 73.85 \\
CoOp \scriptsize{(ICCV2021)}          & 88.33 & 82.26 & 85.19 & 40.44 & 22.30 & 28.75 & 80.60 & 65.89 & 72.51 & 79.44 & 41.18 & 54.24 & 92.19 & 54.74 & 68.69 & 84.69 & 56.05 & 67.46 \\
ATPrompt$_{CoOp}$ \scriptsize{(ICCV2025)} & 88.74 & 87.44 & 88.09 & 40.38 & 27.22 & 32.52 & 80.84 & 68.64 & 74.24 & 80.83 & 45.49 & 58.22 & 90.34 & 59.79 & 71.96 & 84.49 & 64.96 & 73.45 \\
ProGrad \scriptsize{(CVPR2023)}         & 90.37 & 89.59 & 89.98 & 40.54 & 27.57 & 32.82 & 81.26 & 74.17 & 77.55 & 77.35 & 52.35 & 62.45 & 90.11 & 60.89 & 72.67 & 84.33 & 74.94 & 79.35 \\
MaPLe \scriptsize{(CVPR2023)}         & 90.71 & 92.05 & 91.38 & 37.44 & 35.61 & 36.50 & 80.82 & 78.70 & 79.75 & 80.36 & 59.18 & 68.16 & 94.07 & 73.23 & 82.35 & 83.00 & 78.66 & 80.77 \\
PromptSRC \scriptsize{(ICCV2023)}     & 90.67 & 91.53 & 91.10 & 42.73 & 37.87 & 40.15 & 82.67 & 78.47 & 80.52 & 83.37 & 62.97 & 71.75 & 92.90 & 73.90 & 82.32 & 87.10 & 78.80 & 82.74 \\
ProVP \scriptsize{(CVPR2024)}        & 90.32 & 90.91 & 90.61 & 47.08 & 29.87 & 36.55 & 83.14 & 74.71 & 78.73 & 62.11 & 65.53 & 63.77 & \textbf{97.12} & 72.91 & 83.29 & 87.30 & 79.00 & 83.00 \\
TCP \scriptsize{(CVPR2024)}           & 90.57 & 91.37 & 90.97 & 41.97 & 34.43 & 37.83 & 82.63 & 78.20 & 80.35 & 82.77 & 58.07 & 68.25 & 91.63 & 74.73 & 82.32 & 87.13 & 80.77 & 83.83 \\
PromptKD \scriptsize{(CVPR2024)}      & 89.43 & 91.27 & 90.34 & 43.61 & \textbf{39.68} & 41.55 & 82.53 & 80.88 & 81.70 & 82.86 & 69.15 & 75.39 & 92.04 & 71.59 & 80.54 & 86.23 & 80.11 & 83.06 \\
MMRL \scriptsize{(CVPR2025)}          & 90.57 & 91.50 & 91.03 & 46.30 & 37.03 & 41.15 & 83.20 & 79.30 & 81.20 & \textbf{85.67} & 65.00 & 73.82 & 95.60 & 80.17 & 87.21 & \textbf{88.10} & 80.07 & 83.89 \\
TAC \scriptsize{(CVPR2025)}           & \textbf{90.87} & 91.87 & \textbf{91.37} & 44.60 & 37.70 & 40.86 & 83.70 & 80.03 & 81.82 & 83.37 & 64.27 & 72.58 & 94.37 & 82.60 & 88.10 & 88.07 & 81.67 & 84.75 \\
SkipT \scriptsize{(CVPR2025)} & 90.67 & \textbf{92.03} & 91.34 & 45.37 & 37.13 & 40.84 & 82.40 & 79.03 & 80.68 & 83.77 & 67.23 & 74.59 & 92.47 & 83.00 & 87.48 & 87.30 & \textbf{82.47} & 84.81 \\
\midrule
\rowcolor{lightgray} 
\textbf{DeAR (Ours)}                       & 90.10 & 91.90 & 90.93 & \textbf{47.10} & 38.90 & \textbf{42.61} & \textbf{83.82} & \textbf{81.80} & \textbf{82.80} & 83.90 & \textbf{75.60} & \textbf{79.62} & 97.00 & \textbf{87.90} & \textbf{92.22} & 87.90 & 82.10 & \textbf{84.90} \\
\bottomrule
\end{tabular}
}
\label{b2n}
\end{table*}



% \begin{table*}[ht]
% \centering
% \caption{Comparison of DeAR with previous methods on base-to-novel generalization across 11 datasets. Bold values indicate the best results.}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{Method} 
%     & \multicolumn{3}{c|}{Average} 
%     & \multicolumn{3}{c|}{ImageNet} 
%     & \multicolumn{3}{c|}{Caltech101} 
%     & \multicolumn{3}{c|}{OxfordPets}
%     & \multicolumn{3}{c|}{StanfordCars} 
%     & \multicolumn{3}{c}{Flowers102} \\
%  & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM \\
% \midrule
% CLIP \scriptsize{(ICML2021)}          & 69.34 & 74.22 & 71.70 & 72.43 & 68.14 & 70.22 & 96.84 & 94.00 & 95.40 & 91.17 & 97.96 & 94.12 & 63.37 & 74.89 & 68.65 & 72.08 & 77.80 & 74.83 \\
% CoOp \scriptsize{(ICCV2021)}          & 82.69 & 63.22 & 71.66 & 76.47 & 67.88 & 71.92 & 98.01 & 89.81 & 93.73 & 93.67 & 95.29 & 94.47 & 78.12 & 60.40 & 68.13 & 97.60 & 59.67 & 74.06 \\
% ProGrad \scriptsize{(CVPR2023)}         & 82.48 & 70.75 & 76.16 & 77.02 & 66.66 & 71.46 & 98.02 & 93.89 & 95.91 & 95.07 & 97.63 & 96.33 & 77.68 & 68.63 & 72.88 & 95.54 & 71.87 & 82.03 \\
% MaPLe \scriptsize{(CVPR2023)}         & 82.28 & 75.14 & 78.55 & 76.60 & 70.54 & 73.47 & 97.74 & 94.36 & 96.02 & 95.43 & 97.76 & 96.58 & 72.94 & 74.00 & 73.47 & 95.92 & 72.46 & 82.56 \\
% PromptSRC \scriptsize{(ICCV2023)}     & 84.26 & 76.10 & 79.97 & 77.60 & 70.73 & 74.01 & 98.10 & 94.03 & 96.02 & 95.33 & 97.30 & 96.30 & 78.27 & 74.97 & 76.58 & 98.07 & 76.50 & 85.95 \\
% ProVP \scriptsize{(CVPR2024)}        & 85.20 & 73.22 & 78.76 & 75.82 & 69.21 & 72.36 & 98.92 & 94.21 & 96.51 & 95.87 & 97.65 & 96.75 & 80.43 & 67.96 & 73.67 & 98.42 & 72.06 & 83.20 \\
% TCP \scriptsize{(CVPR2024)}           & 84.13 & 75.36 & 79.51 & 77.27 & 69.87 & 73.38 & 98.23 & 94.67 & 96.42 & 94.67 & 97.20 & 95.92 & 80.80 & 74.13 & 77.32 & 97.73 & 75.57 & 85.23 \\
% PromptKD \scriptsize{(CVPR2024)}      & 84.11 & 78.28 & 81.09 & 77.63 & 70.96 & 74.15 & 98.31 & \textbf{96.29} & \textbf{97.29} & 93.42 & 97.44 & 95.39 & 80.48 & \textbf{81.78} & \textbf{81.12} & 98.69 & \textbf{81.91} & \textbf{89.52} \\
% MMRL \scriptsize{(CVPR2025)}          & 85.68 & 77.16 & 81.20 & 77.90 & 71.30 & 74.45 & 98.97 & 94.50 & 96.68 & 95.90 & 97.60 & 96.74 & 81.30 & 75.07 & 78.06 & 98.97 & 77.27 & 86.78 \\
% TAC \scriptsize{(CVPR2025)}           & 85.24 & 77.60 & 81.24 & \textbf{78.57} & 71.03 & 74.61 & 98.57 & 95.27 & 96.89 & 95.93 & \textbf{98.17} & \textbf{97.04} & 81.63 & 74.17 & 77.72 & 97.97 & 76.87 & 86.15 \\
% SkipT \scriptsize{(CVPR2025)} & 85.04 & 77.53 & 81.11 & 77.73 & 70.40 & 73.89 & 98.50 & 95.33 & 96.89 & 95.70 & 97.87 & 96.77 & \textbf{82.93} & 72.50 & 77.37 & 98.57 & 75.80 & 85.70 \\
% \midrule
% \rowcolor{lightgray} % <--- 添加这一行
% \textbf{DeAR (Ours)}                   & \textbf{85.94} & \textbf{79.73} & \textbf{82.72} & 78.12 & \textbf{71.80} & \textbf{74.83} & \textbf{99.00} & 95.80 & 96.95 & \textbf{97.34} & 97.50 & 96.81 & 82.01 & 75.20 & 78.47 & \textbf{99.00} & 78.50 & 87.57 \\
% \bottomrule
% \end{tabular}
% }
% \vspace{0.1cm}

% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{Method} 
%     & \multicolumn{3}{c|}{Food101} 
%     & \multicolumn{3}{c|}{FGVC Aircraft} 
%     & \multicolumn{3}{c|}{SUN397} 
%     & \multicolumn{3}{c|}{DTD}
%     & \multicolumn{3}{c|}{EuroSAT}
%     & \multicolumn{3}{c}{UCF101} \\
%  & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM & Base & Novel & HM \\
% \midrule
% CLIP \scriptsize{(ICML2021)}          & 90.10 & 91.22 & 90.66 & 27.19 & 36.29 & 31.09 & 69.36 & 75.35 & 72.23 & 53.24 & 59.90 & 56.37 & 56.48 & 64.05 & 60.03 & 70.53 & 77.50 & 73.85 \\
% CoOp \scriptsize{(ICCV2021)}          & 88.33 & 82.26 & 85.19 & 40.44 & 22.30 & 28.75 & 80.60 & 65.89 & 72.51 & 79.44 & 41.18 & 54.24 & 92.19 & 54.74 & 68.69 & 84.69 & 56.05 & 67.46 \\
% ProGrad \scriptsize{(CVPR2023)}         & 90.37 & 89.59 & 89.98 & 40.54 & 27.57 & 32.82 & 81.26 & 74.17 & 77.55 & 77.35 & 52.35 & 62.45 & 90.11 & 60.89 & 72.67 & 84.33 & 74.94 & 79.35 \\
% MaPLe \scriptsize{(CVPR2023)}         & 90.71 & 92.05 & 91.38 & 37.44 & 35.61 & 36.50 & 80.82 & 78.70 & 79.75 & 80.36 & 59.18 & 68.16 & 94.07 & 73.23 & 82.35 & 83.00 & 78.66 & 80.77 \\
% PromptSRC \scriptsize{(ICCV2023)}     & 90.67 & 91.53 & 91.10 & 42.73 & 37.87 & 40.15 & 82.67 & 78.47 & 80.52 & 83.37 & 62.97 & 71.75 & 92.90 & 73.90 & 82.32 & 87.10 & 78.80 & 82.74 \\
% ProVP \scriptsize{(CVPR2024)}        & 90.32 & 90.91 & 90.61 & 47.08 & 29.87 & 36.55 & 83.14 & 74.71 & 78.73 & 62.11 & 65.53 & 63.77 & \textbf{97.12} & 72.91 & 83.29 & 87.30 & 79.00 & 83.00 \\
% TCP \scriptsize{(CVPR2024)}           & 90.57 & 91.37 & 90.97 & 41.97 & 34.43 & 37.83 & 82.63 & 78.20 & 80.35 & 82.77 & 58.07 & 68.25 & 91.63 & 74.73 & 82.32 & 87.13 & 80.77 & 83.83 \\
% PromptKD \scriptsize{(CVPR2024)}      & 89.43 & 91.27 & 90.34 & 43.61 & \textbf{39.68} & 41.55 & 82.53 & 80.88 & 81.70 & 82.86 & 69.15 & 75.39 & 92.04 & 71.59 & 80.54 & 86.23 & 80.11 & 83.06 \\
% MMRL \scriptsize{(CVPR2025)}          & 90.57 & 91.50 & 91.03 & 46.30 & 37.03 & 41.15 & 83.20 & 79.30 & 81.20 & \textbf{85.67} & 65.00 & 73.82 & 95.60 & 80.17 & 87.21 & \textbf{88.10} & 80.07 & 83.89 \\
% TAC \scriptsize{(CVPR2025)}           & \textbf{90.87} & 91.87 & \textbf{91.37} & 44.60 & 37.70 & 40.86 & 83.70 & 80.03 & 81.82 & 83.37 & 64.27 & 72.58 & 94.37 & 82.60 & 88.10 & 88.07 & 81.67 & 84.75 \\
% SkipT \scriptsize{(CVPR2025)} & 90.67 & \textbf{92.03} & 91.34 & 45.37 & 37.13 & 40.84 & 82.40 & 79.03 & 80.68 & 83.77 & 67.23 & 74.59 & 92.47 & 83.00 & 87.48 & 87.30 & \textbf{82.47} & 84.81 \\
% \midrule
% \rowcolor{lightgray} % <--- 添加这一行
% \textbf{DeAR (Ours)}                       & 90.10 & 91.90 & 90.93 & \textbf{47.10} & 38.90 & \textbf{42.61} & \textbf{83.82} & \textbf{81.80} & \textbf{82.80} & 83.90 & \textbf{75.60} & \textbf{79.62} & 97.00 & \textbf{87.90} & \textbf{92.22} & 87.90 & 82.10 & \textbf{84.90} \\
% \bottomrule
% \end{tabular}
% }
% \label{b2n}
% \end{table*}

==> sec/cross_dataset.tex <==
% \begin{table*}[ht]
% \centering
% \caption{Comparison of DeAR with previous methods on cross-dataset evaluation. Bold values indicate the best results.}
% \label{tab:cross_dataset_results}
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{llc|ccccccccccc}
% \toprule
% & & \multicolumn{1}{c|}{Source} & \multicolumn{11}{c}{Target} \\
% \cmidrule(lr){3-3} \cmidrule(lr){4-14}
%  &  & \rotatebox{60}{ImageNet} & \rotatebox{60}{Average} & \rotatebox{60}{Caltech101} & \rotatebox{60}{OxfordPets} & \rotatebox{60}{StanfordCars} & \rotatebox{60}{Flowers101} & \rotatebox{60}{Food101} & \rotatebox{60}{FGVC-\newline Aircraft} & \rotatebox{60}{SUN397} & \rotatebox{60}{DTD} & \rotatebox{60}{EuroSAT} & \rotatebox{60}{UCF101} \\
% \midrule
% CoOp       & & 71.51 & 63.88 & 93.70 & 89.14 & 64.51 & 68.71 & 85.30 & 18.47 & 64.15 & 41.92 & 46.39 & 66.55 \\
% MaPLe      &  & 70.72 & 66.30 & 93.53 & 90.49 & 65.57 & 72.23 & 86.20 & 24.74 & 67.01 & 46.49 & 48.06 & 68.69 \\
% PromptSRC  &  & 71.27 & 65.81 & 93.60 & 90.25 & 65.70 & 70.25 & 86.15 & 23.90 & 67.10 & 46.87 & 45.50 & 68.75 \\
% MMRL   & & 72.03 & 67.25 & 94.67 & \textbf{91.43} & 66.10 & 72.77 & 86.40 & 26.30 & 67.57 & 45.90 & 53.10 & 68.27 \\
% TAC & & \textbf{72.77} & 66.53 & 94.53 & 90.67 & 65.30 & 72.20 & 85.83 & 23.53 & 67.63 & \textbf{47.57} & 48.07 & \textbf{70.00} \\
% \midrule
% DeAR   & & 71.50 & \textbf{67.60} & \textbf{95.00} & 91.23 & \textbf{66.70} & \textbf{73.80} & \textbf{86.80} & \textbf{26.50} & \textbf{68.30} & 45.40 & \textbf{53.50} & 68.80 \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

\begin{table*}[ht]
\centering
\caption{Comparison of DeAR with previous methods on cross-dataset evaluation. Bold values indicate the best results.}
\resizebox{\textwidth}{!}{
\begin{tabular}{llc|ccccccccccc}
\toprule
& & \multicolumn{1}{c|}{Source} & \multicolumn{11}{c}{Target} \\
\cmidrule(lr){3-3} \cmidrule(lr){4-14}
 &  & {ImageNet} & {Average} & {Caltech101} & {OxfordPets} & {StanfordCars} & {Flowers102} & {Food101} & {FGVC-\newline Aircraft} & {SUN397} & {DTD} & {EuroSAT} & {UCF101} \\
\midrule
CoOp       & & 71.51 & 63.88 & 93.70 & 89.14 & 64.51 & 68.71 & 85.30 & 18.47 & 64.15 & 41.92 & 46.39 & 66.55 \\
MaPLe      &  & 70.72 & 66.30 & 93.53 & 90.49 & 65.57 & 72.23 & 86.20 & 24.74 & 67.01 & 46.49 & 48.06 & 68.69 \\
PromptSRC  &  & 71.27 & 65.81 & 93.60 & 90.25 & 65.70 & 70.25 & 86.15 & 23.90 & 67.10 & 46.87 & 45.50 & 68.75 \\
MMRL   & & 72.03 & 67.25 & 94.67 & \textbf{91.43} & 66.10 & 72.77 & 86.40 & 26.30 & 67.57 & 45.90 & 53.10 & 68.27 \\
TAC & & \textbf{72.77} & 66.53 & 94.53 & 90.67 & 65.30 & 72.20 & 85.83 & 23.53 & 67.63 & \textbf{47.57} & 48.07 & \textbf{70.00} \\
\midrule
\rowcolor{lightgray} % <--- 添加这一行
\textbf{DeAR (Ours)}   & & 71.50 & \textbf{67.60} & \textbf{95.00} & 91.23 & \textbf{66.70} & \textbf{73.80} & \textbf{86.80} & \textbf{26.50} & \textbf{68.30} & 45.40 & \textbf{53.50} & 68.80 \\
\bottomrule
\end{tabular}
}
\label{tab:cross_dataset_results}
\end{table*}


==> sec/generalization.tex <==
% \begin{table}[ht]
% \centering
% \caption{Comparison of DeAR with previous methods on domainl generalization task. Bold values indicate the best results.}
% \label{tab:domain_gen_results}
% \resizebox{0.4\textwidth}{!}{
% \begin{tabular}{llc|cccc}
% \toprule
% & & \multicolumn{1}{c|}{Source} & \multicolumn{4}{c}{Target} \\
% \cmidrule(lr){3-3} \cmidrule(lr){4-7}
%  &  & ImageNet & -V2 & -S & -A & -R \\
% \midrule
% CoOp        & & 71.51 & 64.20 & 47.99 & 49.71 & 75.21 \\
% MaPLe       & & 70.72 & 64.07 & 49.15 & 50.90 & 76.98 \\
% PromptSRC   & & 71.27 & 64.35 & 49.55 & 50.90 & 77.80 \\
% MMRL    & & 72.03 & 64.47 & 49.17 & 51.20 & 77.53 \\
% TAC & & \textbf{72.77} & 65.97 & \textbf{50.30} & 51.73 & \textbf{78.50} \\
% \midrule
% \textbf{DeAR (Ours)}  & & 71.50 & \textbf{64.87} & 49.50 & \textbf{51.80} & 78.13 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}[ht]
\centering
\caption{Comparison of DeAR with previous methods on domain generalization. Bold values indicate the best results.}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{llc|ccccc}
\toprule
& & \multicolumn{1}{c|}{Source} & \multicolumn{5}{c}{Target} \\
\cmidrule(lr){3-3} \cmidrule(lr){4-8}
 &  & ImageNet & Average & -V2 & -S & -A & -R \\
\midrule
CoOp        & & 71.51 & 59.28 & 64.20 & 47.99 & 49.71 & 75.21 \\
MaPLe       & & 70.72 & 60.28 & 64.07 & 49.15 & 50.90 & 76.98 \\
PromptSRC   & & 71.27 & 60.65 & 64.35 & 49.55 & 50.90 & 77.80 \\
MMRL    & & 72.03 & 60.59 & 64.47 & 49.17 & 51.20 & 77.53 \\
TAC & & \textbf{72.77} & \textbf{61.63} & \textbf{65.97} & \textbf{50.30} & 51.73 & 78.50 \\
\midrule
\rowcolor{lightgray} % <--- 添加这一行
\textbf{DeAR (Ours)}  & & 71.50 & 61.25 & 64.87 & 49.50 & \textbf{51.80} & \textbf{78.83} \\
\bottomrule
\end{tabular}
}
\label{tab:domain_gen_results}
\end{table}

==> sec/head_roles.tex <==
\begin{table*}[t]
\centering
\caption{Representative examples of functionally specialized Attribute Heads identified in the later layers of ViT-B-16. Each head demonstrates a strong and unambiguous focus on a single core visual attribute, as evidenced by its top descriptive phrases.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l|l|l}
\toprule
\textbf{Object Head} & \textbf{Shape Head} & \textbf{Texture Head} & \textbf{Color Head} & \textbf{Location Head} \\
\textbf{(L12, H7)} & \textbf{(L12, H5)} & \textbf{(L11, H5)} & \textbf{(L12, H10)} & \textbf{(L12, H0)} \\
\midrule
- A stick & - A regular octagon & - Delicate embroidery & - An image with cold green tones & - Picture taken in Scotland \\
- A cup & - Rectangular object & - Intricate architectural carving & - Image with a red color & - Photo taken in Barcelona \\
- A bonnet & - A wavy pattern & - Artwork with kaleidoscopic patterns & - A charcoal gray color & - Photo taken in Tokyo, Japan \\
- A trampoline & - Herringbone pattern & - Image with woven basket textures & - Image with a yellow color & - Image taken in South Africa \\
- A shoelace & - A scalene triangle & - Artwork with Mondrian-like grids & - Image with a blue color & - Picture taken in Texas, USA \\
- A bottle & - A polka dot & - Image with calligraphy writing & - A platinum silver color & - Photo taken in Paris, France \\
% - A basket & - Image with a zebra & - Image with calligraphy writing & - Image with a pink color & - Image captured in California \\
% - A violin & - A snail & - Artwork featuring Morse code typography & - Soft pastel tones & - Photo taken in Cairo, Egypt \\
\bottomrule
\end{tabular}%
}
\label{tab:attribute_head_examples_wide}
\end{table*}
